New Bounds for the Vertices of the Integer Hull

The vertices of the integer hull are the integral equivalent to the well-studied basic feasible solutions of linear programs. In this paper we give new bounds on the number of non-zero components -- their support -- of these vertices matching either the best known bounds or improving upon them. While the best known bounds make use of deep techniques, we only use basic results from probability theory to make use of the concentration of measure effect. To show the versatility of our techniques, we use our results to give the best known bounds on the number of such vertices and an algorithm to enumerate them. We also improve upon the known lower bounds to show that our results are nearly optimal. One of the main ingredients of our work is a generalization of the famous Hoeffding bound to vector-valued random variables that might be of general interest.

==> broken.tex <==

\section{Simple bounds}
Remember that the number of inequalities of \eqref{IP:PI} is denoted by $n$. 
Consider any integral solution $p^{*}$ of \eqref{IP:PI} with support
$S=\supp(p^{*})$.
For $t\in \mathbb{Z}^{n}$, let $H_{t}=\{x\in [0,1]^{|S|}\mid A[S]x=t\}$ be the
$t$-th translation of the hyperplane defined by $A[S]$.
Furthermore let $a_{1},\ldots,a_{n}$ be the rows of $A[S]$. 
The following lemma compares $\hyper_{|S|}$ with $A[S]\cdot \hyper_{|S|}$. 
\begin{lemma}\
  
  \begin{enumerate}
  \item $|\hyper_{|S|}|=2^{|S|}$
  \item For each $x\in \hyper_{|S|}$, there is a $t\in \mathbb{Z}^{n}$ with
    $x\in H_{t}$ such that $|t[j]|\leq \lVert a_{j} \rVert_{1}$ for all
    $j=1,\ldots,n$. 
  \item $|A[S]\cdot \hyper_{|S|}|\leq \prod_{j=1}^{n}(2\lVert a_{j} \rVert_{1}+1)$. 
  \end{enumerate}
  
\end{lemma}

\begin{proof}\

  \begin{enumerate}
  \item This is trivially true by definition.
  \item We have $(A[S]x)[j]=\sum_{i=1}^{|S|}a_{j}[i]\cdot x[i]$ and thus
    $-\lVert a_{j} \rVert_{1} \leq (A[S]x)[j]\leq \lVert a_{j} \rVert_{1}$, as $x[i]\in
    \{0,1\}$. 
  \item This directly follows from the second statement of the lemma. 
  \end{enumerate}
\end{proof}

Hence, if $2^{|S|}> \prod_{j=1}^{n}(2\lVert a_{j} \rVert_{1}+1)$, there are two
different points $y_{1},y_{2}\in \hyper_{|S|}$ such that $A[S]y_{1} =
A[S]y_{2}$.
 Now, define $x\in \mathbb{Z}^{d}$ with
  \begin{align*}
    x[i] =
    \begin{cases}
      y_{1}[i]-y_{2}[i] & i\in S\\
      0 & \text{else}.
    \end{cases}
  \end{align*}
  This gives a non-zero vector $x$ and using Lemma~\ref{lem:eisenbrand:shmonin}
  implies that $p^{*}$ is not an integer vertex.
  The inequality $2^{|S|}>\prod_{j=1}^{n}(\lVert a_{j} \rVert_{1}+1)$ can be
  rewritten as $|S|\geq \sum_{j=1}^{n}\log(\lVert a_{j} \rVert_{1}+1)$.
  Clearly, $\sum_{j=1}^{n}\log(\lVert a_{j} \rVert_{1}+1) \leq n\cdot
  \log(|S|\cdot \lVert A[S] \rVert_{\infty}+1)$ and we obtain the following
  lemma.
  \begin{lemma}
    If $|S|> n\cdot
  \log(|S|\cdot \lVert A[S] \rVert_{\infty}+1)$, the solution $p^{*}$ is not an
  integer vertex. 
  \end{lemma}
  

% \subsection{Characterizing the Vertices}

% We will now characterize the integer vertices of the knapsack polytope.
% Instead of looking only at completely integral points of the hypercube lying on
% the vertices of the hypercube, we will also look at near-integral points that
% lie on the edges of the hypercube. 
% Consider any integral solution $p^{*}$ of \eqref{IP:PI} with support
% $S=\supp(p^{*})$. 
% Let $a[S]$ be the subvector of $a$ projected to the elements indexed by $S$.
% Without loss of generality, we assume that $S=\{1,\ldots,|S|\}$. 
% We say that a vector $x\in [0,1]^{|S|}$ is \emph{near-integral}, if there is a
% set $R\subseteq S$, an index $j\not\in R$, and an integer $k\leq a[j]$  with
% \begin{align*}
%   x[i] =
%   \begin{cases}
%     k/a[j] & i=j\\
%     1 & i\in R\\
%     0 & \text{else}.
%   \end{cases}
% \end{align*}
% We denote this vector as $x_{(R,j,k)}$ and the set of all such points as
% $\mathrm{Near}$, i.\,e., $\mathrm{Near}=\{x_{(R,j,k)}\mid R\subseteq S,
% j\not\in R, k\in \{0,\ldots,a[j]\}\}$. 
% For $t\in \mathbb{Z}$, let $H_{t}=\{x\in [0,1]^{|S|}\mid a[S]x=t\}$ be the
% $t$-th translation of the hyperplane defined by $a[S]$. 

% The following lemma shows that it is sufficient to find two similar
% near-integral points to use Lemma~\ref{lem:eisenbrand:shmonin}.
% \begin{lemma}
%   \label{lem:kp:similar}
%   If two different vectors $x_{(R,j,k)}, x_{(R',j',k)}\in \mathrm{Near}$ with
%   $x_{(R,j,k)},x_{(R',j',k)}\in H_{t}$ and $x_{(R,j,0)}\neq x_{(R',j',0)}$
%   exist, $p^{*}$ is not an integer vertex.
% \end{lemma}
% \begin{proof}
%   Let $x_{(R,j,k)}, x_{(R',j',k)}\in \mathrm{Near}$ be two different vectors with
%   $x_{(R,j,k)},x_{(R',j',k)}\in H_{t}$. 
%   It is easy to see that $x_{(R,j,0)},x_{(R',j',0)}\in H_{t-k}$.
%   Now, define $x\in \mathbb{Z}^{d}$ with
%   \begin{align*}
%     x[i] =
%     \begin{cases}
%       x_{(R,j,0)}[i]-x_{(R',j',0)}[i] & i\leq |S|\\
%       0 & \text{else}.
%     \end{cases}
%   \end{align*}
%   Now, $ax=0$ and $-|p^{*}_{i}|\leq x_{i}\leq |p^{*}_{i}|$ for all
%   $i=1,\ldots,d$.
%   The assumption $x_{(R,j,0)}\neq x_{(R',j',0)}$ implies that $x$ is not zero. 
%   Lemma~\ref{lem:eisenbrand:shmonin} then implies that $p^{*}$ is not a vertex
%   of the integer polytope. 
% \end{proof}

 

% We will now compare the relation of these near-integral vectors with the
% hyperplanes defined by $a[S]$. 

% The following lemma shows the strong relation between the translations of $a[S]$
% and the near-integral points.

% \begin{lemma}
%   \label{lem:near:properties}
% It holds that
% \begin{enumerate}
% \item for all $x\in \mathrm{Near}$, there is a $t\in \mathbb{Z}$ such
%   that $x\in H_{t}$ with $-\lVert a[S] \rVert_{1}\leq t\leq \lVert a[S] \rVert_{1} $, and
% \item there are exactly $2^{|S|-1}\cdot (\lVert a[S] \rVert_{1}+1)$ vectors in
%   $\mathrm{Near}$. 
% \end{enumerate}
% \end{lemma}
% \begin{proof}\

%   \begin{enumerate}
%   \item For $x=x_{(R,j,k)}\in \mathrm{Near}$, we have
%     \begin{align*}
%       a[S]\cdot x = \sum_{i\in R}a_{i}+ a_{j}\cdot (k/a_{j})=\sum_{i\in R}a_{i}+a_{j}. 
%     \end{align*}
%     Hence, $-\lVert a[S] \rVert_{1}\leq a[S]\cdot x \leq \lVert a[S] \rVert_{1}$.
%   \item For each $j\in \{1,\ldots,|S|\}$, there are exactly $\binom{|S|-1}{r}$
%     subsets $R$ of size $r$ that do not contain $j$. For each of those subsets,
%     we can choose $a[j]$ possibilities for a value $k > 0$. Hence, there are
%     \begin{align*}
%       \sum_{j=1}^{|S|}\sum_{r=0}^{|S|-1}\binom{|S|-1}{r}\cdot a[j] = 2^{|S|-1}\cdot \lVert a[S] \rVert_{1}
%     \end{align*}
%     such choices with $k > 0$. For $k=0$, there are exactly $2^{|S|-1}$ possible
%     subsets for $R$. Hence, there are exactly $2^{|S|-1}\cdot (\lVert a[S]
%     \rVert_{1}+1)$ elements in $\mathrm{Near}$. 
%   \end{enumerate}
% \end{proof}

% Combining Lemma~\ref{lem:kp:similar} and Lemma~\ref{lem:near:properties} gives
% the following Theorem.

% \begin{theorem}
%   \label{thm:kp:supp_bound}
%   If $|S| > \log_{2}(|S|\cdot \lVert a[S] \rVert_{\infty}+1)+2$, the vector $p^{*}$ is not a vertex of the integer polytope. 
% \end{theorem}
% \begin{proof}
%   Lemma~\ref{lem:near:properties} shows that all $2^{|S|-1}(\lVert a[S]
%   \rVert_{1}+1)$ near-integral points are distributed on the $2\lVert a[S]
%   \rVert_{1}+1$ hyperplanes. 
%   The pidgeonhole principle then implies that there is a hyperplane $H_{t}$ such
%   that $|H_{t}\cap \mathrm{Near}| \geq \frac{2^{|S|-1}(\lVert a[S]
%     \rVert_{1}+1)}{2\lVert a[S] \rVert_{1}+1}\geq \frac{2^{|S|-1}(\lVert a[S]
%     \rVert_{1}+1)}{2(\lVert a[S] \rVert_{1}+1)} = 2^{|S|-2}$.
%   Furthermore, there is some value $k\in \{0,\ldots,\lVert a[S]
%   \rVert_{\infty}\}$ such that $|\{x_{(R,j,k)}\mid R\subsetneq S, j\not\in
%   R\}\cap H_{t}|\geq 2^{|S|-2}/(\lVert a[S] \rVert_{\infty})$.
%   For each set $R$, there are at most $|S|$ different choices for $j\not\in R$.
%   Hence, if $2^{|S|-2}/(\lVert a[S] \rVert_{\infty}) > |S|$, there are two
%   points $x_{(R,j,k)},x_{(R',j',k)}\in H_{t}$ such that $x_{(R,j,0)}\neq
%   x_{(R',j',0)}$. 
%     Lemma~\ref{lem:kp:similar} then implies that $p^{*}$ is not a vertex of the
%   integer polytope. 
% \end{proof}

